Safe-Embed: Unveiling the Safety-Critical Knowledge of Sentence Encoders

Despite the impressive capabilities of Large Language Models (LLMs) in various tasks, their vulnerability to unsafe prompts remains a critical issue. These prompts can lead LLMs to generate responses on illegal or sensitive topics, posing a significant threat to their safe and ethical use. Existing approaches attempt to address this issue using classification models, but they have several drawbacks. With the increasing complexity of unsafe prompts, similarity search-based techniques that identify specific features of unsafe prompts provide a more robust and effective solution to this evolving problem. This paper investigates the potential of sentence encoders to distinguish safe from unsafe prompts, and the ability to classify various unsafe prompts according to a safety taxonomy. We introduce new pairwise datasets and the Categorical Purity (CP) metric to measure this capability. Our findings reveal both the effectiveness and limitations of existing sentence encoders, proposing directions to improve sentence encoders to operate as more robust safety detectors. Our code is available at https://github.com/JwdanielJung/Safe-Embed.

==> table/CP_average_results.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{l|c|c}
        \hline
        \textbf{Model} & \textbf{AVG} & \textbf{Median} \\
        \hline
        \hline
        sentence-bert-all & 0.443 & 0.438 \\
        sentence-bert-paraphrase & 0.412 & 0.394 \\ 
        sup-simcse & 0.360 & 0.353 \\
        unsup-simcse & \underline{0.327} & \underline{0.320} \\
        st5-base & 0.435 & 0.449 \\
        st5-large & 0.453 & 0.457 \\
        st5-xl & 0.448 & 0.476 \\
        st5-xxl & 0.460 & 0.476 \\
        text-embedding-3-large & \textbf{0.461} & \textbf{0.481} \\
        llm2vec & 0.439 & 0.435 \\
        \hline
    \end{tabular}
    \caption{Average and median value of all categories' CP in each sentence encoder models. The text-embedding-v3 has the highest score(\textbf{bold}) and the unsup-simce has lowest score (\underline{line})}.
    \label{tab:avg cp table}
\end{table}


==> table/category_jaccard.tex <==
\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\textbf{Types of Harm} & \textbf{Size} &\textbf{R1} & \textbf{R2} & \textbf{RL} & \textbf{Jaccard}\\ \hline
Adult Content & 28 & 0.140 & 0.034 & 0.136 & 0.073 \\ \hline
Chatbot treated as Human & 50 & 0.164 & 0.038 & 0.147 & 0.094 \\ \hline
Disinfo Campaigns & 40 & 0.227 & 0.078 & 0.217 & 0.106 \\ \hline
Disseminate Misinformation & 63 & 0.132 & 0.020 & 0.116 & 0.037 \\ \hline
False, Misleading Info & 92 & 0.083 & 0.012 & 0.077 & 0.043 \\ \hline
Hate Speech & 53 & 0.129 & 0.034 & 0.127 & 0.076 \\ \hline
Illegal Activities & 132 & 0.193 & 0.068 & 0.189 & 0.108 \\ \hline
Mental Health Crisis & 67 & 0.163 & 0.047 & 0.154 & 0.083 \\ \hline
Privacy Leaks (Org/Gov) & 136 & 0.128 & 0.033 & 0.124 & 0.070 \\ \hline
Privacy Leaks (Personal) & 112 & 0.194 & 0.032 & 0.191 & 0.101 \\ \hline
Stereotypes & 95 & 0.164 & 0.032 & 0.160 & 0.091 \\ \hline
Unethical Actions & 71 & 0.218 & 0.065 & 0.195 & 0.110 \\ \hline
\end{tabular}
}
\caption{The statistics of dataset and the results of the ROUGE F1 scores (R1, R2, RL) and Jaccard Similarity between sentence pairs within same unsafe category. A higher ROUGE score and a Jaccard Similarity imply higher lexical overlaps. Each category has low lexical score in all scores, which means all the query in the category is not lexically similar. We use the short version of "types of harm" names because it is too long.}

 % Please find details about the metrics used here in Appendix B
\label{table:categoric_lexical_sim}
\end{table}

==> table/donotanswer_stats.tex <==
\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|c|}
\hline
\textbf{Types of harm} & \textbf{size} \\ \hline
Adult Content & 28 \\ \hline
Chatbot treated as Human & 50 \\ \hline
Disinfo Campaigns & 40 \\ \hline
Disseminate Misinformation & 63 \\ \hline
False, Misleading information & 92 \\ \hline
Hate Speech & 53 \\ \hline
Illegal Activities & 132 \\ \hline
Mental Health Crisis & 67 \\ \hline
Privacy Leaks (Org/Gov) & 136 \\ \hline
Privacy Leaks (Personal) & 112 \\ \hline
Stereotypes & 95 \\ \hline
Unethical Actions & 71 \\ \hline
\end{tabular}
}
\caption{The size of different "types of harm" in Do-not-answer dataset}
\label{table:stats_don}
\end{table}

==> table/xstest_result.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{1.3}
\centering
\resizebox{\textwidth}{!}{
\tiny
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
\hline
                  & homonyms & figurative language & target & context & definitions & group & action & history & privacy public & privacy fictional & Average \\
sbert-all         & 0.394    & 0.296                & 0.494  & 0.653   & 0.534       & 0.514 & 0.385  & 0.698   & 0.396           & 0.511              & 0.4875  \\
sbert-paraphrase  & 0.39     & 0.29                 & 0.475  & 0.62    & 0.575       & 0.529 & 0.405  & 0.72    & 0.427           & 0.558              & 0.4989  \\
sup-simcse        & 0.532    & 0.476                & 0.561  & 0.634   & 0.594       & 0.587 & 0.499  & 0.736   & 0.439           & 0.527              & 0.5585  \\
unsup-simcse      & 0.492    & 0.476                & 0.513  & 0.625   & 0.616       & 0.527 & 0.43   & 0.676   & 0.428           & 0.552              & 0.5335  \\
st5-base          & 0.462    & 0.395                & 0.499  & 0.641   & 0.535       & 0.613 & 0.407  & 0.668   & 0.499           & 0.585              & 0.5304  \\
st5-large         & 0.403    & 0.364                & 0.517  & 0.597   & 0.475       & 0.575 & 0.344  & 0.585   & 0.405           & 0.525              & 0.479   \\
st5-xl            & 0.388    & 0.325                & 0.492  & 0.593   & 0.471       & 0.524 & 0.321  & 0.57    & 0.368           & 0.514              & 0.4566  \\
st5-xxl           & 0.37     & 0.298                & 0.442  & 0.562   & 0.467       & 0.522 & 0.302  & 0.524   & 0.348           & 0.508              & 0.4343  \\
text-embedding-3-large & 0.424    & 0.369                & 0.479  & 0.613   & 0.473       & 0.528 & 0.367  & 0.599   & 0.29            & 0.443              & 0.4585  \\
llm2vec           & 0.361    & 0.336                & 0.427  & 0.429   & 0.436       & 0.432 & 0.325  & 0.654   & 0.275           & 0.36               & 0.4035  \\

\hline
\end{tabular}
}
\caption{xstest result}

\end{table*}

